ORC Layout: Adaptive GUI Layout with OR-Constraints

We propose a novel approach for constraint-based graphical user interface (GUI) layout based on OR-constraints (ORC) in standard soft/hard linear constraint systems. ORC layout unifies grid layout and flow layout, supporting both their features as well as cases where grid and flow layouts individually fail. We describe ORC design patterns that enable designers to safely create flexible layouts that work across different screen sizes and orientations. We also present the ORC Editor, a GUI editor that enables designers to apply ORC in a safe and effective manner, mixing grid, flow and new ORC layout features as appropriate. We demonstrate that our prototype can adapt layouts to screens with different aspect ratios with only a single layout specification, easing the burden of GUI maintenance. Finally, we show that ORC specifications can be modified interactively and solved efficiently at runtime.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-sigconf-authordraft.tex \
	samples/sample-sigconf-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-sigconf-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done

samples/sample-manuscript.pdf \
samples/sample-acmsmall.pdf \
samples/sample-acmlarge.pdf \
samples/sample-acmtog.pdf: samples/samplebody-journals.tex

samples/sample-sigconf.pdf \
samples/sample-sigconf-authordraft.pdf \
samples/sample-sigconf-xelatex.pdf \
samples/sample-sigplan.pdf \
samples/sample-sigchi.pdf: samples/samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean
	$(RM) $(PDF) samples/*-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.


==> text/_FormatReference.tex <==
\section{Introduction}

The \textit{proceedings} are the records of a conference.\footnote{This
  is a footnote}  ACM seeks
to give these conference by-products a uniform, high-quality
appearance.  To do this, ACM has some rigid requirements for the
format of the proceedings documents: there is a specified format
(balanced double columns), a specified set of fonts (Arial or
Helvetica and Times Roman) in certain specified sizes, a specified
live area, centered on the page, specified size of margins, specified
column width and gutter size.

\section{The Body of The Paper}
Typically, the body of a paper is organized into a hierarchical
structure, with numbered or unnumbered headings for sections,
subsections, sub-subsections, and even smaller sections.  The command
\texttt{{\char'134}section} that precedes this paragraph is part of
such a hierarchy.\footnote{This is a footnote.} \LaTeX\ handles the
numbering and placement of these headings for you, when you use the
appropriate heading commands around the titles of the headings.  If
you want a sub-subsection or smaller part to be unnumbered in your
output, simply append an asterisk to the command name.  Examples of
both numbered and unnumbered headings will appear throughout the
balance of this sample document.

Because the entire article is contained in the \textbf{document}
environment, you can indicate the start of a new paragraph with a
blank line in your input file; that is why this sentence forms a
separate paragraph.

\subsection{Type Changes and {\itshape Special} Characters}

We have already seen several typeface changes in this sample.  You can
indicate italicized words or phrases in your text with the command
\texttt{{\char'134}textit}; emboldening with the command
\texttt{{\char'134}textbf} and typewriter-style (for instance, for
computer code) with \texttt{{\char'134}texttt}.  But remember, you do
not have to indicate typestyle changes when such changes are part of
the \textit{structural} elements of your article; for instance, the
heading of this subsection will be in a sans serif\footnote{Another
  footnote here.  Let's make this a rather long one to see how it
  looks.} typeface, but that is handled by the document class file.
Take care with the use of\footnote{Another footnote.}  the
curly braces in typeface changes; they mark the beginning and end of
the text that is to be in the different typeface.

You can use whatever symbols, accented characters, or non-English
characters you need anywhere in your document; you can find a complete
list of what is available in the \textit{\LaTeX\ User's Guide}
\cite{Lamport:LaTeX}.

\subsection{Math Equations}
You may want to display math equations in three distinct styles:
inline, numbered or non-numbered display.  Each of
the three are discussed in the next sections.

\subsubsection{Inline (In-text) Equations}
A formula that appears in the running text is called an
inline or in-text formula.  It is produced by the
\textbf{math} environment, which can be
invoked with the usual \texttt{{\char'134}begin\,\ldots{\char'134}end}
construction or with the short form \texttt{\$\,\ldots\$}. You
can use any of the symbols and structures,
from $\alpha$ to $\omega$, available in
\LaTeX~\cite{Lamport:LaTeX}; this section will simply show a
few examples of in-text equations in context. Notice how
this equation:
\begin{math}
  \lim_{n\rightarrow \infty}x=0
\end{math},
set here in in-line math style, looks slightly different when
set in display style.  (See next section).

\subsubsection{Display Equations}
A numbered display equation---one set off by vertical space from the
text and centered horizontally---is produced by the \textbf{equation}
environment. An unnumbered display equation is produced by the
\textbf{displaymath} environment.

Again, in either environment, you can use any of the symbols
and structures available in \LaTeX\@; this section will just
give a couple of examples of display equations in context.
First, consider the equation, shown as an inline equation above:
\begin{equation}
  \lim_{n\rightarrow \infty}x=0
\end{equation}
Notice how it is formatted somewhat differently in
the \textbf{displaymath}
environment.  Now, we'll enter an unnumbered equation:
\begin{displaymath}
  \sum_{i=0}^{\infty} x + 1
\end{displaymath}
and follow it with another numbered equation:
\begin{equation}
  \sum_{i=0}^{\infty}x_i=\int_{0}^{\pi+2} f
\end{equation}
just to demonstrate \LaTeX's able handling of numbering.

\subsection{Citations}
Citations to articles~\cite{bowman:reasoning,
clark:pct, braams:babel, herlihy:methodology},
conference proceedings~\cite{clark:pct} or maybe
books \cite{Lamport:LaTeX, salas:calculus} listed
in the Bibliography section of your
article will occur throughout the text of your article.
You should use BibTeX to automatically produce this bibliography;
you simply need to insert one of several citation commands with
a key of the item cited in the proper location in
the \texttt{.tex} file~\cite{Lamport:LaTeX}.
The key is a short reference you invent to uniquely
identify each work; in this sample document, the key is
the first author's surname and a
word from the title.  This identifying key is included
with each item in the \texttt{.bib} file for your article.

The details of the construction of the \texttt{.bib} file
are beyond the scope of this sample document, but more
information can be found in the \textit{Author's Guide},
and exhaustive details in the \textit{\LaTeX\ User's
Guide} by Lamport~\shortcite{Lamport:LaTeX}.

This article shows only the plainest form
of the citation command, using \texttt{{\char'134}cite}.

Some examples.  A paginated journal article \cite{Abril07}, an enumerated
journal article \cite{Cohen07}, a reference to an entire issue \cite{JCohen96},
a monograph (whole book) \cite{Kosiur01}, a monograph/whole book in a series (see 2a in spec. document)
\cite{Harel79}, a divisible-book such as an anthology or compilation \cite{Editor00}
followed by the same example, however we only output the series if the volume number is given
\cite{Editor00a} (so Editor00a's series should NOT be present since it has no vol. no.),
a chapter in a divisible book \cite{Spector90}, a chapter in a divisible book
in a series \cite{Douglass98}, a multi-volume work as book \cite{Knuth97},
an article in a proceedings (of a conference, symposium, workshop for example)
(paginated proceedings article) \cite{Andler79}, a proceedings article
with all possible elements \cite{Smith10}, an example of an enumerated
proceedings article \cite{VanGundy07},
an informally published work \cite{Harel78}, a doctoral dissertation \cite{Clarkson85},
a master's thesis: \cite{anisi03}, an online document / world wide web
resource \cite{Thornburg01, Ablamowicz07, Poker06}, a video game (Case 1) \cite{Obama08} and (Case 2) \cite{Novak03}
and \cite{Lee05} and (Case 3) a patent \cite{JoeScientist001},
work accepted for publication \cite{rous08}, 'YYYYb'-test for prolific author
\cite{SaeediMEJ10} and \cite{SaeediJETC10}. Other cites might contain
'duplicate' DOI and URLs (some SIAM articles) \cite{Kirschmer:2010:AEI:1958016.1958018}.
Boris / Barbara Beeton: multi-volume works as books
\cite{MR781536} and \cite{MR781537}.

A couple of citations with DOIs: \cite{2004:ITE:1009386.1010128,
  Kirschmer:2010:AEI:1958016.1958018}.

Online citations: \cite{TUGInstmem, Thornburg01, CTANacmart}.


\subsection{Tables}
Because tables cannot be split across pages, the best
placement for them is typically the top of the page
nearest their initial cite.  To
ensure this proper ``floating'' placement of tables, use the
environment \textbf{table} to enclose the table's contents and
the table caption.  The contents of the table itself must go
in the \textbf{tabular} environment, to
be aligned properly in rows and columns, with the desired
horizontal and vertical rules.  Again, detailed instructions
on \textbf{tabular} material
are found in the \textit{\LaTeX\ User's Guide}.

Immediately following this sentence is the point at which
Table~\ref{tab:freq} is included in the input file; compare the
placement of the table here with the table in the printed
output of this document.

\begin{table}
  \caption{Frequency of Special Characters}
  \label{tab:freq}
  \begin{tabular}{ccl}
    \toprule
    Non-English or Math&Frequency&Comments\\
    \midrule
    \O & 1 in 1,000& For Swedish names\\
    $\pi$ & 1 in 5& Common in math\\
    \$ & 4 in 5 & Used in business\\
    $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
  \bottomrule
\end{tabular}
\end{table}

To set a wider table, which takes up the whole width of the page's
live area, use the environment \textbf{table*} to enclose the table's
contents and the table caption.  As with a single-column table, this
wide table will ``float'' to a location deemed more desirable.
Immediately following this sentence is the point at which
Table~\ref{tab:commands} is included in the input file; again, it is
instructive to compare the placement of the table here with the table
in the printed output of this document.


\begin{table*}
  \caption{Some Typical Commands}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    Command &A Number & Comments\\
    \midrule
    \texttt{{\char'134}author} & 100& Author \\
    \texttt{{\char'134}table}& 300 & For tables\\
    \texttt{{\char'134}table*}& 400& For wider tables\\
    \bottomrule
  \end{tabular}
\end{table*}
% end the environment with {table*}, NOTE not {table}!

It is strongly recommended to use the package booktabs~\cite{Fear05}
and follow its main principles of typography with respect to tables:
\begin{enumerate}
\item Never, ever use vertical rules.
\item Never use double rules.
\end{enumerate}
It is also a good idea not to overuse horizontal rules.


\subsection{Figures}

Like tables, figures cannot be split across pages; the best placement
for them is typically the top or the bottom of the page nearest their
initial cite.  To ensure this proper ``floating'' placement of
figures, use the environment \textbf{figure} to enclose the figure and
its caption.

This sample document contains examples of \texttt{.eps} files to be
displayable with \LaTeX.  If you work with pdf\LaTeX, use files in the
\texttt{.pdf} format.  Note that most modern \TeX\ systems will convert
\texttt{.eps} to \texttt{.pdf} for you on the fly.  More details on
each of these are found in the \textit{Author's Guide}.

\begin{figure}
\includegraphics{fly}
\caption{A sample black and white graphic.}
\end{figure}

\begin{figure}
\includegraphics[height=1in, width=1in]{fly}
\caption{A sample black and white graphic
that has been resized with the \texttt{includegraphics} command.}
\end{figure}


As was the case with tables, you may want a figure that spans two
columns.  To do this, and still to ensure proper ``floating''
placement of tables, use the environment \textbf{figure*} to enclose
the figure and its caption.  And don't forget to end the environment
with \textbf{figure*}, not \textbf{figure}!

\begin{figure*}
\includegraphics{flies}
\caption{A sample black and white graphic
that needs to span two columns of text.}
\end{figure*}


\begin{figure}
\includegraphics[height=1in, width=1in]{rosette}
\caption{A sample black and white graphic that has
been resized with the \texttt{includegraphics} command.}
\end{figure}

\subsection{Theorem-like Constructs}

Other common constructs that may occur in your article are the forms
for logical constructs like theorems, axioms, corollaries and proofs.
ACM uses two types of these constructs:  theorem-like and
definition-like.

Here is a theorem:
\begin{theorem}
  Let $f$ be continuous on $[a,b]$.  If $G$ is
  an antiderivative for $f$ on $[a,b]$, then
  \begin{displaymath}
    \int^b_af(t)\,dt = G(b) - G(a).
  \end{displaymath}
\end{theorem}

Here is a definition:
\begin{definition}
  If $z$ is irrational, then by $e^z$ we mean the
  unique number that has
  logarithm $z$:
  \begin{displaymath}
    \log e^z = z.
  \end{displaymath}
\end{definition}

The pre-defined theorem-like constructs are \textbf{theorem},
\textbf{conjecture}, \textbf{proposition}, \textbf{lemma} and
\textbf{corollary}.  The pre-defined de\-fi\-ni\-ti\-on-like constructs are
\textbf{example} and \textbf{definition}.  You can add your own
constructs using the \textsl{amsthm} interface~\cite{Amsthm15}.  The
styles used in the \verb|\theoremstyle| command are \textbf{acmplain}
and \textbf{acmdefinition}.

Another construct is \textbf{proof}, for example,

\begin{proof}
  Suppose on the contrary there exists a real number $L$ such that
  \begin{displaymath}
    \lim_{x\rightarrow\infty} \frac{f(x)}{g(x)} = L.
  \end{displaymath}
  Then
  \begin{displaymath}
    l=\lim_{x\rightarrow c} f(x)
    = \lim_{x\rightarrow c}
    \left[ g{x} \cdot \frac{f(x)}{g(x)} \right ]
    = \lim_{x\rightarrow c} g(x) \cdot \lim_{x\rightarrow c}
    \frac{f(x)}{g(x)} = 0\cdot L = 0,
  \end{displaymath}
  which contradicts our assumption that $l\neq 0$.
\end{proof}

\section{Conclusions}
This paragraph will end the body of this sample document.
Remember that you might still have Acknowledgments or
Appendices; brief samples of these
follow.  There is still the Bibliography to deal with; and
we will make a disclaimer about that here: with the exception
of the reference to the \LaTeX\ book, the citations in
this paper are to articles which have nothing to
do with the present subject and are used as
examples only.
%\end{document}  % This is where a 'short' article might terminate



\appendix
%Appendix A
\section{Headings in Appendices}
The rules about hierarchical headings discussed above for
the body of the article are different in the appendices.
In the \textbf{appendix} environment, the command
\textbf{section} is used to
indicate the start of each Appendix, with alphabetic order
designation (i.e., the first is A, the second B, etc.) and
a title (if you include one).  So, if you need
hierarchical structure
\textit{within} an Appendix, start with \textbf{subsection} as the
highest level. Here is an outline of the body of this
document in Appendix-appropriate form:
\subsection{Introduction}
\subsection{The Body of the Paper}
\subsubsection{Type Changes and  Special Characters}
\subsubsection{Math Equations}
\paragraph{Inline (In-text) Equations}
\paragraph{Display Equations}
\subsubsection{Citations}
\subsubsection{Tables}
\subsubsection{Figures}
\subsubsection{Theorem-like Constructs}
\subsubsection*{A Caveat for the \TeX\ Expert}
\subsection{Conclusions}
\subsection{References}
Generated by bibtex from your \texttt{.bib} file.  Run latex,
then bibtex, then latex twice (to resolve references)
to create the \texttt{.bbl} file.  Insert that \texttt{.bbl}
file into the \texttt{.tex} source file and comment out
the command \texttt{{\char'134}thebibliography}.
% This next section command marks the start of
% Appendix B, and does not continue the present hierarchy
\section{More Help for the Hardy}

Of course, reading the source code is always useful.  The file
\path{acmart.pdf} contains both the user guide and the commented
code.

\begin{acks}
  The authors would like to thank Dr. Yuhua Li for providing the
  MATLAB code of the \textit{BEPS} method.

  The authors would also like to thank the anonymous referees for
  their valuable comments and helpful suggestions. The work is
  supported by the \grantsponsor{GS501100001809}{National Natural
    Science Foundation of
    China}{http://dx.doi.org/10.13039/501100001809} under Grant
  No.:~\grantnum{GS501100001809}{61273304}
  and~\grantnum[http://www.nnsf.cn/youngscientists]{GS501100001809}{Young
    Scientists' Support Program}.

\end{acks}


==> text/_OLD_3_System.tex <==
\setlength{\abovedisplayskip}{-10pt}%
\setlength{\belowdisplayskip}{0pt}%
\setlength{\abovedisplayshortskip}{-10pt}%
\setlength{\belowdisplayshortskip}{0pt}%


\section{ORC Editor}
ORC Editor looks like a standard GUI builder which consists a control panel, a canvas panel
%(Figure \ref{fig:orc_editor}), 
and a property panel.
 %for different layout patterns (shown in the ORC patterns section)
ORC layouts can be edited using the control panel or drag and drop operations in the canvas panel.
Through the control panel, the user can resize the canvas, add new widgets, resize existing ones, and remove widgets. In the canvas panel, the user can interactively rearrange, resize, or delete widgets via drag-and-drop operations. The ORC layout algorithm automatically solves the constraint system after each adjustment made by the user. To keep the layout solvable, we follow ALE \cite{zeidler2013auckland}, by detecting, highlighting, and disabling conflicting constraints.

% removed for now.
% \begin{figure}[H]
% \includegraphics[width=\columnwidth]{figures/1_ORCEditor.pdf}
% \caption{(a) In the control panel, we allow end-users to resize the canvas, and insert, delete, or resize various types of widgets. (b) In the canvas, we render the widgets with the optimal layout with soft, hard, and alternative constraints. The designer can also rearrange, resize, or delete widgets directly in the canvas.
% }
% \label{fig:orc_editor}
% \end{figure}

\subsection{Solving a System with OR-constraints}

The naïve approach to solve a system with OR-constraints is to try all solutions. For very small systems, this might be feasible but does not scale well: for every OR-constraints with two parts,
%(only one part needs to be true to satisfy the OR-constraints), 
there are two potential solutions. This number grows exponentially, {\em e.g.}, with only ten OR-constraints there are 1024 potential solutions that need to be evaluated. This naïve strategy quickly becomes impractical.

OR-constrained systems are a subset of SMT (Satisfiability Modulo Theory) problems. Hence, instead of an explicit solver algorithm, we use Z3 \cite{de2008z3}, which is a very efficient SMT solver. Z3 typically scored in the yearly SMT competitions\footnote{SMT competitions: \url{smtcomp.org}} during the last decade.
One of the key insights of our work is that SMT solvers can be used to solve GUI layouts with OR-constraints. Z3 supports first-order logic, but also linear constraints with priorities commonly used for GUI layout. As such, it has the ability to solve specifications with disjunctive sets of constraint alternatives, which makes it an ideal tool to solve a system of constraints that includes OR-constraints. We have not seen failures of convergence with Z3. Z3 has previously been proposed for solving formalized CSS layout specifications \cite{panchekha2016automated}. However, to the best of our knowledge, it has not been used for general GUI layout before.

Re-solving the constraint system iteratively after each adjustment in the canvas layout can be very time-consuming. If we re-solve the entire constraint system after each change to the canvas layout, this may dramatically slow down the speed for producing a good layout result. To produce layout results dynamically and efficiently at runtime, computations need to be efficient. By reusing parts of the previous solution, Z3 supports incremental solving, {\em i.e.}, it produces a result faster, if the current constraint system is similar to the previous one. Hence, in our ORC Editor, instead of re-creating the whole constraint system after each adjustment in the layout, we remove unsatisfied constraints from the previously solved system and add new constraints. Thus, our approach re-solves only part of the new constraint system based on the previous results and achieves better performance. 

\subsection{ORC Layouts for screen rotation}

OR-constraints can unify flow layouts and grid layouts, which opens up options for layouts to work across screen rotations and cases where grid and flow layouts individually fail. The ORC Editor gives developers the interactive tools to define flexible layouts more easily by combining the power of grid and flow layouts. It enables designers to seamlessly deal with screen rotations with a single layout specification.

For instance, neither grid nor flow layouts can deal with the case in Figure \ref{fig:rotation_example2} through a single layout specification that involves only a single layout method, {\em i.e.}, not a combination of multiple layout methods. 
There are three high-level widgets (labeled areas) in the canvas layout: tea, block, and clock, denoted as [a], [b], and [c] respectively. Inside block [b], we have three low-level widgets: image, document, and chart, denoted as [1], [2], and [3]. We create the following OR-constraint to solve this problem. 

\begin{align*}
C_\OR &=
\left( 
    \left(
        \MB_\WIDTH \leftarrow \sum_{i=1}^3 \MI_\WIDTH 
    \right)
    \wedge
    \left(
        \MB_\HEIGHT \leftarrow \max_{i=1,2,3} \MI_\HEIGHT 
    \right)
\right)
\\
 & 
{\bf OR} \left(
    \left(
        \MB_\HEIGHT \leftarrow \sum_{i=1}^3 \MI_\HEIGHT 
    \right)
    \wedge
    \left(
        \MB_\WIDTH \leftarrow \max_{i=1,2,3} \MI_\WIDTH 
    \right)
\right)
\end{align*}

\begin{figure}[H]
\includegraphics[scale=0.25]{figures/rotation_ex1.png}
\caption{An ORC layout with a single layout specification for horizontal and vertical rotation. Classic methods, such as flow and grid layouts, can realize such a layout only through a hierarchy of layouts or code that switches layout managers depending on the window aspect ratio.}
\label{fig:rotation_example1}
\end{figure}

If the solver yields a solution corresponding to the first soft constraint in this OR-constraint, then the layout will place the labels horizontally in the block, otherwise vertically.

Next, we demonstrate a more practical use case of an ORC layout for device rotation in Fig. \ref{fig:rotation_example2}. This layout contains a menu, a file explorer panel, a main view for code editing, and a control panel with widgets for searching, replacing, and console debugging. It uses OR-constraints similar to the previous example. 
%Similar to the previous example, we group the three blocks into a common control panel and add the OR-constraint to the constraint-based system to determine if they should be placed horizontally or vertically. %In this case, we also add two additional hard constraints to ensure the menu is always at the top and the explorer is always on the left:


% \begin{align*}
%     \M{menu}_\WIDTH &\leftarrow \M{canvas}_\WIDTH \\
%     \M{explorer}_\TOP &\leftarrow \M{canvas}_\HEIGHT - \M{explorer}_\HEIGHT
% \end{align*}


\begin{figure}[t]
\includegraphics[scale=0.4]{figures/rotation_ex2.png}
\caption{A practical use case of ORC layouts for dealing with different device orientations. Note that the entire layout changes from horizontal to vertical while the inner layout of the control panel changes the opposite way. }
\label{fig:rotation_example2}
\end{figure}

In our prototype, we solve the OR-constraints system through a Python backend and Z3. We transfer the results back to the Javascript front end and place all widgets at the computed positions and sizes.

\section{ORC Layouts}
In ORC layouts, and as is common for constraint-based layouts, the minimum, preferred, and maximum size of each widget and the relationships among widgets are all defined by constraints. In addition to hard and soft constraints, the constraint system for ORC layout also contains OR-constraints. OR-constraints enable the designer to specify multiple alternative constraints, only one of which needs to be met. 

A simple example for an alternative constraint is a toolbar that is on the left side in landscape mode but is repositioned to the top (or bottom) of the screen in portrait mode. An OR-constraint can express this kind of layout specification in a simple manner. The designer only needs to specify both alternative constraints joined with an OR-clause. Thus, with OR-constraints, a single layout specification can support many different screen sizes and aspect ratios.

We define OR-constraints through a mixture of hard and soft constraints. The whole OR-constraint is defined as a hard constraint, while each part of the OR-constraint is an additional and independent soft constraint. %For instance, let’s say ``A or B or C'' is an OR-constraint we add to the constraint system. When the solver tries to solve the constraint system, at least one of A, B, and C must be satisfied, but not all of them have to be satisfied. Hence, an OR-constraint “A or B or C” is instantiated as a hard “A or B or C” and “A”, “B”, and “C” as 3 additional, independent soft constraints.

Some individual soft-constrained parts of an OR-constraint can be given higher priority than others through weights, which defines the level of importance or priority of that part.
%Larger weights should be attached to more important soft constraints, so that these constraints have higher priorities. 
For example, in the OR-constraint ``to the right OR at the beginning of next row'', we prefer to place the current widget to the right of the previous one. Thus, we attach a larger, {\em e.g}, double, weight to the part ``to the right''.

\subsection{Flexibility}

 When a user specifies a layout, the system creates the corresponding constraints with default parameters. Through instantiation of our pre-defined flow-layout constraints, we substantially reduce the complexity presented to the user. The user can modify parameters to meet more specialized requirements. 
 %Constraints for the size of the canvas and widgets can be modified in the control panel.
 %shown in Figure \ref{fig:orc_editor}.
 Below, we show parts of the property panel for layout patterns, through which users can {\em e.g.}, choose where they want to place the toolbar, whether widgets are placed and ordered horizontally or vertically, or whether widgets in different toolbars are connected. Each option instantiates a pre-defined set of constraints. Through this mechanism users have the freedom to choose which functionality they want to apply to the layout without having to deal with constraints directly.

\subsection{ORC Layout Edit Operations}

Our ORC Editor supports all standard edit operations, such as resize, move, insert, and delete. These operations can be activated through the control panel or interactively in the canvas. The GUI builder creates the constraint-based layout and displays the result after solving the constraint system. After each change made in the canvas layout, the system re-solves automatically. 
%The canvas layout can be resized by modifying the entries ``width'' and ``height'' in the control panel or by dragging of the bottom right corner of the canvas layout. 
For efficiency, the solver re-solves a layout only when the user finishes a drag operation. 
%Then the system will update the placement and size of all the widgets in the canvas layout according to the solution of the constraint system. 
\subsection{Layout Editing Examples}

% Here we discuss what happens when an ORC layout is edited.
%In Figure \ref{fig:resizing_layout}, after we drag the bottom right corner of the canvas layout to change the size of the window, the ORC layout will automatically rearrange all the widgets in the window. In essence, this is a flow layout implemented via constraints.

\subsubsection{Resizing the Canvas}
Figure \ref{fig:resizing_layout} shows a flow layout implemented via OR-constraints being interactively resized.

\begin{figure}[t]
\includegraphics[scale=0.15]{figures/4_Resizing_Layout.png}
\caption{Window resizing for a ORC flow layout}
% \caption{After the user resize the canvas layout, the first three widgets remain in the first row, while the other widgets are automatically arranged to the next row due to the OR-constraint which implements a flow layout behavior.}
\label{fig:resizing_layout}
\end{figure}

\subsubsection{Moving}
%\textcolor{red}{Wolfgang: This subsection and the following two do not read that well. The algorithms described here are not truly general - they are (too) specific to the widgets. It would already be better if button was replaced by a ``constant-sized'' widget or some similar phrase. Ideally, this and the following 2 sections should not be specific to the type of widget and the specific constraint in the layout, instead it should handle the moving, resizing, inserting/deleting of widgets - regardless if our constraint-based flow-layout is used or not. See, e.g., the ALE paper to get an idea how this might be described better.}

%Moving is an edit operation which is performed directly in the canvas layout. 
A move operation involves dragging a widget and then dropping it to the new position. 
Moving a widget can not only change the positions of widgets, but also sometimes cause resizing of widgets or regrouping widgets into different ``blocks'' {\em e.g.}, aligning the moved button with other buttons.
%Moving a widget not only alters the position of the moved widget, but also affects the positions of other widgets. How to determine the new positions of all the affected widgets is a critical challenge we need to address. Sometimes such a move may also cause resizing of widgets. 
%Each moving operation can cause three types of results. A trivial move operation would just change the positions of widgets. The moved widget, along with all the widgets located between its original position and its updated position could have changed positions after the move operation. When we move a button, the situation will be much more complicated since we need to check whether there are other buttons around the target position. If so, we can align them in the same column and handle the combination of these buttons as a block in the layout. That means if later a widget is placed at a position around this button block, it would probably be placed to the right or to the left of the block instead of separating these buttons (unless it is a button, it fits in the block). (Figure \ref{fig:moving})

When there are several widgets in a block, the width and height of that widget should be the maximum length and height of the buttons within the block and preferably be the same as the previous block/widget in the same row. Here, we show how constraints can be used to specify such a layout for a block. First, we define two hard constraints:

\begin{align*}
    \M{block}_\WIDTH &\leftarrow \max_{i=1,\cdots,n} \left( \M{button~i}_\WIDTH \right) \\
    \M{block}_\HEIGHT &\geq \sum_i \M{button~i}_\HEIGHT 
\end{align*}

where $n$ is the number of buttons in the block. This is complemented by a soft constraint:

\begin{equation*}
    \M{block}_\HEIGHT \leftarrow \M{prev~block}_\HEIGHT
\end{equation*}

\begin{figure}[H]
\includegraphics[scale=0.2]{figures/6_Moving.png}
\caption{Illustration of a move operations in the ORC Editor. The first step causes resizing of the ``pie chart''. The second step only changes the position of the moved widget. The third step combines two buttons into a block since the moved widget “No” button can be combined with the “Yes” button.}
\label{fig:moving}
\end{figure}

\subsubsection{Resizing Widgets}

%Widgets in the canvas layout can be resized by modifying the width or height entry of a widget in the control panel or using drag and drop operation directly in the canvas layout. 
Resizing a widget modifies the hard constraints for the preferred size of the widget. Similar to moving a widget, resizing one widget can also change the constraints for other ones.

%If the left boundary or the right boundary of a widget is dragged, then the width of the widget will be changed and similarly for the top/bottom boundaries, which change the height. If the corner of a widget is dragged, then both the width and the height of the widget will be modified. (e.g. Figure \ref{fig:resizing_widgets})

\begin{figure}[t]
\includegraphics[scale=0.15]{figures/5_Resizing_Widgets.png}
\caption{Widget resizing}
\label{fig:resizing_widgets}
\end{figure}

\subsubsection{Inserting and Deleting}

The users can insert new widgets into the canvas. %via the control panel by defining the position, contents, and preferred size of the new widget. 
If a resizable widget, {\em {\em e.g.}}, a text area, is inserted, six new soft constraints for min/pref/max widths and heights respectively will be added to the constraint system. If the new widget cannot be resized ({\em {\em e.g.}}, a button), then two hard constraints for width and height will be added. 

Our ORC Editor also allows the designer to delete a widget via the control panel or by dragging a widget outside of the window. For most cases, deleting a widget just means moving all the widgets after it into the top left of the empty space (Figure \ref{fig:deleting1}). However, the OR-constraints we add guarantee that if a widget (or sometimes several widgets) is at the start of a row, then some widgets might move to the end of the previous row, if possible. Some instances of widget deletions are more challenging. For instance, as shown in Figure \ref{fig:deleting2}, the removed widget might be located between two different button blocks. In this case, they can be combined to a single block after deletion.

\begin{figure}[t]
\includegraphics[scale=0.15]{figures/7_Deleting1.png}
\caption{After removing the “photos” icon, the buttons “Yes” and “No” are moved to the first row due to the OR-constraint “to the right”.}
\label{fig:deleting1}
\end{figure}

\begin{figure}[t]
\includegraphics[scale=0.15]{figures/8_Deleting2.png}
\caption{After removing the “document” icon, the button “No” is aligned into the same column as the “Yes” button. They are combined to a single block after deletion.}
\label{fig:deleting2}
\end{figure}


\section{ORC Layout Patterns}

Here we present the constraints for several of our new layout patterns. To our knowledge no current layout mechanism or editor can deal with the shown examples, except through multiple layout specifications or code.

\subsection{Mixed layout specifications}

Previous layout managers often focus on solving a single type of layout. The use of OR-constraints makes it possible to mix different types of constraints and layout specifications. For example, a ``to the right OR at the start of the next row below'' constraint between each successive pair of widgets enables ORC layouts to unify flow and grid-bag layouts. With such a unified layout, the designer only needs to create a single layout specification for both landscape and portrait for common layouts.

%We prefer a widget to be to the right of the previous widget rather than be positioned at the start of the next row below, so we express this through appropriate priorities: the soft constraint representing ``to the right'' only needs to be given much higher priority than the soft constraint representing ``at the start of the next row below''. In this case, since ``to the right'' has been attached a higher weight, it has higher priority and is more important.

In the following, we assume that all widgets are ordered in the layout. We denote the $i$-th widget as $\MI$ and the set of all widgets as $W$. 
For each widget $\MI \in W$, we define its left \& top position, width, and height as $\MI_\LEFT$,$\MI_\TOP$, $\MI_\WIDTH$, $\MI_\HEIGHT$ respectively. We use "$M  \leftarrow N$" to denote “Let M be N”.
The soft constraint ``to the right'', $C_{Right}$, is  formulated as:

\begin{align*}
    C_{Right} & = \left( \MI_\LEFT \leftarrow \MII_\LEFT+ \MII_\WIDTH \right) \\
    & \wedge \left( \MI_\TOP \leftarrow \MII_\TOP \right)
\end{align*}

The soft constraint ``at the start of the next row below'', $C_{NextRow}$, is formulated as:

\begin{align*}
C_{NextRow} &= (\MI_\LEFT \leftarrow 0)  \wedge \\
 & \left( \MI_\TOP\geq \MJ_\TOP + \MJ_\HEIGHT, \forall j < i, \MJ \in W  \right)
\wedge \\
& \left( \bigvee_j \MI_\TOP \leftarrow \MJ_\TOP + \MJ_\HEIGHT, \forall j < i, \MJ \in W \right)
\end{align*}

The OR-constraint $C_{Horizontal}$ is then a hard constraint with a disjunction of the two soft constraints ``to the right'' and ``at the start of the next row below'':

\begin{equation*}
    C_{Horizontal} = C_{Right}\ \ OR\ \ C_{NextRow}
\end{equation*}


\begin{figure}[t]
\includegraphics[scale=0.35]{figures/h_v.jpg}
\caption{The horizontal window uses a ``to the right OR at the start of the next row", while the vertical one has an OR-constraint ``to the bottom OR at the start of the next column''.}
\label{fig:h_v}
\end{figure}

We also implemented an OR-constraint for ``to the bottom OR at the start of the next column'', which places widgets in columns, and where each widget prefers to be placed to the bottom of the previous one. 

% In this case, the OR-constraint $C_{Vertical}$ is a hard constraint which is the disjunction of the two soft constraints ``to the bottom'' $C_{Bottom}$ and ``at the start of the next column'' $C_{NextCol}$:

% \begin{equation*}
%     C_{Vertical} = C_{Bottom}\ \ OR\ \ C_{NextCol}
% \end{equation*}

As shown in Figure \ref{fig:h_v}, users can choose whether they want a horizontal of vertical flow layout, which switches between these two patterns.



\subsection{Cross-cutting Layout Pattern}

\begin{figure}[t]
\includegraphics[scale=0.4]{figures/cross_cutting.jpg}
\caption{Cross-cutting layout pattern: a content pane surrounded by a top toolbar with a horizontal flow layout and a left toolbar with a vertical flow layout. }
\label{fig:cross_cutting}
\end{figure}

In the cross-cutting layout pattern, each widget in the top toolbar has the constraint ``to the right OR at the beginning of next row'' and each in the left toolbar has the constraint ``to the bottom OR at the beginning of next column''. The toolbars automatically transform into multiple rows/columns as the screen gets smaller. The widgets in the toolbars can be resized to the same to get a nicer result.

\subsection{Connected Cross-cutting Layout Pattern}

\begin{figure}[t]
\includegraphics[scale=0.38]{figures/connected_cross_cutting.jpg}
\caption{Connected cross-cutting layout pattern: cross-cutting layout pattern with widgets in the toolbars connected.}
\label{fig:connected_cross_cutting}
\end{figure}

The connected cross-cutting layout pattern is a generalization, where the areas are connected so that widgets can move between the toolbar areas to fit the screen size better. We compute the most suitable number of widgets in the top toolbar. ($t_{best} = window\_width\ /\ widget\_width$). If the original number of widgets in the top toobar $t$ is smaller than $t_{best}$, then we move the first $t_{best}-t$ widgets in the left toolbar to the top one. Otherwise, move the first $t-t_{best}$ widgets in the top toolbar to the left one. Users can use the property panel to choose whether they want toolbars to be connected.

\subsection{Balanced Flow Layout Pattern}

\begin{figure}[t]
\includegraphics[scale=0.38]{figures/balanced.jpg}
\caption{Balanced flow layout pattern: The toolbar contains 6 widgets. When the widgets in the toolbar are broken into rows, each row can only have 1, 2, 3, or 6 widgets.}
\label{fig:balanced}
\end{figure}


When the widgets in the toolbar are broken into rows, each row can only have a predefined number of widgets (a factor of the number of the widgets in the toolbar). We compute a set of all the factors of the number of the widgets in the toolbar. According to the window size, we get a preferred size of the top toolbar area and then a preferred number of rows in the top toolbar. We pick the closest number $c$ in the factor set, resize the widgets ,and place $t/c$ widgets in each row. 
%This functionality cannot be handled by current GUI editors and other layouts. %I said this above already, deleted as redundant.

\subsection{Alternative Position Layout Pattern}

\begin{figure}[t]
\includegraphics[scale=0.38]{figures/alternative.jpg}
\caption{Alternative position layout pattern: the toolbar can be placed on the top OR to the left.}
\label{fig:alternative}
\end{figure}

With this simple OR-constraint, a top toolbar can be changed to be a left toolbar when the screen size changes or vice versa.
% Users can also use the property panel to modify the position of the toolbar.

\subsection{Widget Alternative Layout Pattern}

If a window does not have enough space, some widgets can have alternative representations to save space. For instance, List Boxes can be replaced by Option Menus. We express this through constraints as follows, where weight of (1) > (2):\\

 $[size(ListBox) == widgetSize(ListBox)$
 
 \qquad \qquad \qquad $\land$ $size(OptionMenu) == 0 \quad (1)]$
 
 \qquad \qquad \qquad  \qquad \qquad $OR$

$[size(ListBox) == 0$ 

 \quad $\land$ $size(OptionMenu) == widgetSize(OptionMenu) \quad (2)]$\\


\subsection{Optional Layout Pattern}
When a window is made smaller, some widgets can be made optional. An example is the ribbon menu in MS Word, where buttons disappear if there is not enough space in the window. The OR-constraint ''the widget has zero size OR nonzero size'' realizes this functionality. 

For each widget in ribbon menu, we assign a weight to it. Widgets with larger weights have higher priorities. Thus, when the window gets smaller, widgets with lower weights disappear before those with higher weights. We use the following constraints to implement this:\\
   $$ size == widgetSize\ OR\ size == 0$$
For widgets with high priority, $size ==  widgetSize$ is a hard constraint. For widgets with medium priority, $size ==  widgetSize$ is a soft constraint with a large weight, and $size == 0$ is a soft constraint with a small weight $A$. For widgets with low priority, $size ==  widgetSize$ is a soft constraint with a large weight, and $size == 0$ is a soft constraint with a small weight $B$,
where weight $A$ > weight $B$.

The example in Figure \ref{fig:optional} shows both the widget alternative and optional functionalities. It demonstrates how the ribbon menu changes as the window gets smaller. In Figure \ref{fig:ribbon_menu}, ``High'', ``Medium'', ``Low'' represent high, medium, low weights. Widgets in the ribbon menu disappear according to their weights when the window gets smaller. In the bottom part, list boxes and radio buttons are replaced by option menus to save space in the window.

\begin{figure}[t]
\includegraphics[scale=0.25]{figures/ribbon_menu.jpg}
\caption{In a ribbon menu, each widget is assigned a weight.}
\label{fig:ribbon_menu}
\end{figure}

\begin{figure}[t]
\includegraphics[width=\columnwidth]{figures/optional.jpg}
\caption{a) Here there is enough space to show all the widgets in the window. b) Medium Size: Widgets with low weight disappear. c) Small Size: Widgets with medium and low weights disappear. Both radio buttons and the list box are replaced by option menus to save space.}
\label{fig:optional}
\end{figure}


\subsection{Flowing Widgets Around a Fixed one}

\begin{figure}[t]
  \includegraphics[scale=0.3]{figures/flowing.jpg}
  \caption{Left: Flow layout with OR-constraints.  The position of the "SIGGRAPH" image is fixed and all the other widgets flow around it. The size of the flowing widgets adjusts to fill up space to align the margins  (on the right). Right: Flow layout without OR-constraints.}
  \label{fig:around}
\end{figure}

An OR-constraint system can even deal with the case of flowing widgets around a fixed one, {\em e.g.}, similar to placing a picture on a page of text and flowing text around it. As shown in Fig. \ref{fig:around} (right), with simple flow layouts a fixed widget would necessitate splitting the window into 4 parts and widgets would flow in each part separately, which results in an undesirable outcome.
However, with OR-constraints, we can flow widgets around the fixed one without splitting the window into parts. The OR-constraint system can solve the whole window at the same time to arrive at a much more pleasing result and even resize widgets to avoid ``ragged right'' margins.

If a widget is above or below the fixed widget, then it has the OR-constraint ``to the right of the previous widget OR at the beginning of next row'' as usual. When a row of widgets overlaps with the rows occupied by the fixed widget, this will cause a row break to prevent overlap. In essence, the fixed widget the cuts the rows into two parts. Algorithm \ref{alg:around} shows how we implemented this layout.

\begin{algorithm}

    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    
\SetAlgoLined


first widget $\rightarrow$ top left corner

\If {overlap} {
first widget $\rightarrow$ after fixed widget}

\If {current widget is above or below the fixed widget} {
    	current\_left == prev\_right {\bf OR} current $\rightarrow$ next\_row 
    	\textcolor{red}{\ (hard)}
        }
\If {current widget shares any row with the fixed widget}
{
    \textcolor{blue}{\tcp {break over rows to prevent overlap}}
    \If {there is enough space for current widget in this row} 
    {
        current\_top == prev\_top \textcolor{red}{\ (hard)}\\
        \If {enough space between previous widget and fixed widget} {
            current\_left == prev\_right
            \textcolor{red}{\ (hard)}
        } \Else {
             current\_left == fixed\_right
            \textcolor{red}{\ (hard)}
        }
    }
    \Else{
	    current $\rightarrow$ next\_row\\	 
    	\If {enough space between previous widget and fixed widget} {
            current\_left == left\_boundary
            \textcolor{red}{\ (hard)}
        }
    	\Else {
            current\_left == fixed\_right
            \textcolor{red}{\ (hard)}
        }
    }
}

current\_top == prev\_top \textcolor{red}{\ (soft with high weight)}

current $\rightarrow$ next\_row\textcolor{red}{\ (soft with low weight)}


\caption{Flowing Widgets Around a Fixed one}
 
\label{alg:around}
\end{algorithm}

Document layout methods also address this case, but through completely different methods. Compared with previous document layout methods, our method does not need to define different sets of constraints for different cases. For example, the Adaptive Grid-Based Document Layout proposed by Jacobs et al. \cite{Jacobs2003document} uses adaptive layout templates to implement similar functionality. With their method, each template needs a set of constraints while with our OR-constraints, all cases can be solved using the same constraint system.




\subsection{Implementation and Evaluation}

We implemented the ORC editor in Python 2.7 with Tkinter, a GUI library for Python. We use the Z3-solver, a SMT solver library \cite{de2008z3} from Microsoft Research to solve the constraint system constructed in constraint-based layouts. We use the default WMax optimization algorithm in Z3 for weighted soft constraint problems \cite{nieuwenhuis2006wmax}.

Efficiency plays a vital role in solving constraint-based systems. We measured the execution time of the ORC layout solver for different editing operations (insert, delete, move, and resize) with different numbers of constraints. For each condition, we measure the average execution time of 10 runs. We conduct the experiments on a laptop with an Intel i5 CPU. As shown in Table 1, when the number of constraints is less than 175, our method can efficiently solve the most common cases in less than one second on this average machine.
For deployment, one could cache solved layouts for typical devices to improve performance. Note that for insert, delete, and move, our ORC Editor incrementally updates the constraint system, which saves approximately 40\%-86\% of the computation time for 5 widgets, and around 30\%-48\% of the time for 20 widgets. In contrast, a resize operation typically requires a complete rebuild of the entire constraint system, which is costlier.

\begin{table}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/table.jpg}
    \caption{Average solving times with ORC layout (in seconds) for different number of constraints and different operations. (“Resize” in this table means resizing specific widgets). In our experiments, we used horizontal flow layout with the OR-constraint "to the right OR at the beginning of next line" and the sizes of widgets are determined by their min/pref/max constraints.}
    \label{tbl:timing}
\end{table}

For more complex cases, our method could take advantage of hierarchical layouts to efficiently solve a new layout in under one second. %The solving time can be reduced by decomposing UIs into hierarchical layouts. 
For example, smaller widgets could be contained in larger bounding boxes, and the layout of individual boxes could be solved efficiently in parallel. 
